CodeKGC: Code Language Model for Generative Knowledge Graph Construction

Current generative knowledge graph construction approaches usually fail to capture structural knowledge by simply flattening natural language into serialized texts or a specification language. However, large generative language model trained on structured data such as code has demonstrated impressive capability in understanding natural language for structural prediction and reasoning tasks. Intuitively, we address the task of generative knowledge graph construction with code language model: given a code-format natural language input, the target is to generate triples which can be represented as code completion tasks. Specifically, we develop schema-aware prompts that effectively utilize the semantic structure within the knowledge graph. As code inherently possesses structure, such as class and function definitions, it serves as a useful model for prior semantic structural knowledge. Furthermore, we employ a rationale-enhanced generation method to boost the performance. Rationales provide intermediate steps, thereby improving knowledge extraction abilities. Experimental results indicate that the proposed approach can obtain better performance on benchmark datasets compared with baselines. Code and datasets are available in https://github.com/zjunlp/DeepKE/tree/main/example/llm.

==> figures/old/codex.tex <==
\begin{figure}[t]
 \centering
 \begin{tikzpicture} 
 \begin{axis}[
 enlargelimits=0.7,
 legend style={at={(0.5,-0.25)},
anchor=north,legend columns=-1},
 symbolic x coords={Serialized Prompt, Structural Prompt},
 xtick=data,
 ybar=5pt,% configures `bar shift'
 bar width=15pt,
 width=8.4cm, height=4.5cm,
 nodes near coords,
 nodes near coords align={vertical},
 nodes near coords style={font=\tiny},
 font=\small,
 grid=major,
 ]
 \addplot[fill=brown!40!white,draw=brown] coordinates {
  (Serialized Prompt, 85.3)
  (Structural Prompt, 77.6)
 };
 \addplot [fill=black!40!white,draw=black] coordinates {
  (Serialized Prompt, 79.3)
  (Structural Prompt, 90.6)
 };
  \addplot [fill=orange!40!white,draw=orange] coordinates {
  (Serialized Prompt, 24.3)
  (Structural Prompt, 40.6)
 };
 \legend{GPT, Codex-GPT, CodeRel}
 \end{axis}
 \end{tikzpicture}
 \caption{Performance Comparison.}
\end{figure}

==> figures/old/codex_prompt_ade.tex <==
% \documentclass[letterpaper]{article} % 
% \usepackage{pgfplots} % 画折线图
% \usepackage{scalefnt} %用于设置字体

% \definecolor{color1}{RGB}{145,30,180}
% \definecolor{color2}{RGB}{245,130,48}
% \definecolor{color3}{RGB}{230,25,75}

% \begin{document}
	
	\begin{figure*}[h] %插入图片
		\centering %图片居中
		\resizebox{1.8\columnwidth}{!}{  %用于修改图片大小
			\begin{tikzpicture} %tikz图片
			\scalefont{0.7} %设置字体大小
			\begin{axis}[
			sharp plot, %控制线的风格
			title=Serialized Prompt,%图像标题
			xmode=normal,% 控制坐标轴为线性
%		ymode=log,% 控制坐标轴为对数
			xlabel=Number of In-context Examples, %x坐标名
			% ylabel=y, %y坐标名
			width=8cm, height=5cm,  %设置长和宽
			xmin=5,xmax=20,  % 设置x坐标范围
			ymin=0, ymax=80,  % 设置y坐标范围
			xtick={5,10,15,20}, %指定x轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			ytick={0, 15,30,45,60,75}, %指定y轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			xlabel near ticks, % 设置x坐标名位置靠近折线图
			ylabel near ticks, % 设置y坐标名位置靠近折线图
			ymajorgrids=true, % 启用/禁用 [公式] 轴上刻度线位置上的网格线
			grid style=dashed, % 设置网格线格式
			legend style={at={(0.9,1.1)},anchor=south}, % 设置标签位置
%			legend columns=3, %设置标签列数
%			legend pos=north west, % 设置折线对应标签的位置
%			legend style={nodes={scale=0.6, transform shape}},  % 设置折线标签的格式
			]
			%画第一条线，semithick设置线的粗细为0.6pt，mark是折线标示形状，options是mark形状的大小 ， olive!50!white是颜色，coordinates中包含要绘制的点的坐标
			\addplot+[semithick,mark=x,mark options={scale=0.6}, color=color1] plot coordinates { 
				(5,35.71)
				(10,38.99)
				(15,36.31)
				(20,42.19)
			};
			% \addlegendentry{text-davinci-002}%第一条线标签	
			%画第二条线
			\addplot+[semithick,mark options={scale=0.3}, color=color2] plot coordinates {
				(5,50.74)
				(10,53.33)
				(15,56.67)
				(20,53.75)
			};
			% \addlegendentry{code-davinci-002} %第二条线标签
			%画第三条线
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(5,64.33)
				(10,59.05)
				(15,63.81)
				(20,71.25)
			};
			% \addlegendentry{text-davinci-002} %第三条线标签
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(5,23.33)
				(10,13.05)
				(15,23.81)
				(20,44.25)
			};
			% \addlegendentry{code-CodeRel} 
			\end{axis}   
			\end{tikzpicture}


			\begin{tikzpicture} %tikz图片
			\scalefont{0.7} %设置字体大小
			\begin{axis}[
			sharp plot, %控制线的风格
			title=Code Prompt,%图像标题
			xmode=normal,% 控制坐标轴为线性
%		ymode=log,% 控制坐标轴为对数
			xlabel=Number of In-context Examples, %x坐标名
			% ylabel=y, %y坐标名
			width=8cm, height=5cm,  %设置长和宽
			xmin=5,xmax=20,  % 设置x坐标范围
			ymin=0, ymax=80,  % 设置y坐标范围
			xtick={5,10,15,20}, %指定x轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			ytick={0, 15,30,45,60,75}, %指定y轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			xlabel near ticks, % 设置x坐标名位置靠近折线图
			ylabel near ticks, % 设置y坐标名位置靠近折线图
			ymajorgrids=true, % 启用/禁用 [公式] 轴上刻度线位置上的网格线
			grid style=dashed, % 设置网格线格式
			legend style={at={(0.9,1.1)},anchor=south}, % 设置标签位置
%			legend columns=3, %设置标签列数
%			legend pos=north west, % 设置折线对应标签的位置
%			legend style={nodes={scale=0.6, transform shape}},  % 设置折线标签的格式
			]
			%画第一条线，semithick设置线的粗细为0.6pt，mark是折线标示形状，options是mark形状的大小 ， olive!50!white是颜色，coordinates中包含要绘制的点的坐标
			\addplot+[semithick,mark=x,mark options={scale=0.6}, color=color1] plot coordinates { 
				(5,35.71)
				(10,38.99)
				(15,36.31)
				(20,42.19)
			};
			% \addlegendentry{text-davinci-002}%第一条线标签	
			%画第二条线
			\addplot+[semithick,mark options={scale=0.3}, color=color2] plot coordinates {
				(5,50.74)
				(10,53.33)
				(15,56.67)
				(20,53.75)
			};
			% \addlegendentry{code-davinci-002} %第二条线标签
			%画第三条线
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(5,64.33)
				(10,59.05)
				(15,63.81)
				(20,71.25)
			};
			% \addlegendentry{text-davinci-002} %第三条线标签
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(5,23.33)
				(10,13.05)
				(15,23.81)
				(20,44.25)
			};
			% \addlegendentry{code-CodeRel} 
			\end{axis}   
			\end{tikzpicture}

  }
		\caption{Analysis of Different  Prompt in ADE } % 设置caption
		\label{fig:label}  % 设置用于reference的label
	\end{figure*}

% \end{document}


==> figures/old/codex_prompt_conll04.tex <==
% \documentclass[letterpaper]{article} % 
% \usepackage{pgfplots} % 画折线图
% \usepackage{scalefnt} %用于设置字体

% \definecolor{color1}{RGB}{145,30,180}
% \definecolor{color2}{RGB}{245,130,48}
% \definecolor{color3}{RGB}{230,25,75}

% \begin{document}
	
	\begin{figure*}[h] %插入图片
		\centering %图片居中
		\resizebox{1.8\columnwidth}{!}{  %用于修改图片大小
			\begin{tikzpicture} %tikz图片
			\scalefont{0.7} %设置字体大小
			\begin{axis}[
			sharp plot, %控制线的风格
			title=serilized prompt,%图像标题
			xmode=normal,% 控制坐标轴为线性
%		ymode=log,% 控制坐标轴为对数
			xlabel=x, %x坐标名
			ylabel=y, %y坐标名
			width=8cm, height=5cm,  %设置长和宽
			xmin=0,xmax=20,  % 设置x坐标范围
			ymin=0, ymax=80,  % 设置y坐标范围
			xtick={0,5,10,15,20}, %指定x轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			ytick={0, 15,30,45,60,75}, %指定y轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			xlabel near ticks, % 设置x坐标名位置靠近折线图
			ylabel near ticks, % 设置y坐标名位置靠近折线图
			ymajorgrids=true, % 启用/禁用 [公式] 轴上刻度线位置上的网格线
			grid style=dashed, % 设置网格线格式
			legend style={at={(0.9,1.1)},anchor=south}, % 设置标签位置
%			legend columns=3, %设置标签列数
%			legend pos=north west, % 设置折线对应标签的位置
%			legend style={nodes={scale=0.6, transform shape}},  % 设置折线标签的格式
			]
			
			%画第一条线，semithick设置线的粗细为0.6pt，mark是折线标示形状，options是mark形状的大小 ， olive!50!white是颜色，coordinates中包含要绘制的点的坐标
			\addplot+[semithick,mark=x,mark options={scale=0.6}, color=color1] plot coordinates { 
				(0,66.58)
				(5,35.71)
				(10,38.99)
				(15,36.31)
				(20,42.19)
			};
			\addlegendentry{text-davinci-002}%第一条线标签
			
			%画第二条线
			\addplot+[semithick,mark options={scale=0.3}, color=color2] plot coordinates {
				(0,71.79)
				(5,50.74)
				(10,53.33)
				(15,56.67)
				(20,53.75)
			};
			\addlegendentry{code-davinci-002} %第二条线标签
			
			%画第三条线
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(0,72.53)
				(5,64.33)
				(10,59.05)
				(15,63.81)
				(20,71.25)
			};
			\addlegendentry{text-davinci-002} %第三条线标签

			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(0,32.53)
				(5,23.33)
				(10,13.05)
				(15,23.81)
				(20,44.25)
			};
			\addlegendentry{code-CodeRel} 

			\end{axis}
			\end{tikzpicture}

			\begin{tikzpicture} %tikz图片
			\scalefont{0.7} %设置字体大小
			\begin{axis}[
			sharp plot, %控制线的风格
			title=code prompt,%图像标题
			xmode=normal,% 控制坐标轴为线性
%		ymode=log,% 控制坐标轴为对数
			xlabel=x, %x坐标名
			ylabel=y, %y坐标名
			width=8cm, height=5cm,  %设置长和宽
			xmin=0,xmax=20,  % 设置x坐标范围
			ymin=0, ymax=80,  % 设置y坐标范围
			xtick={0,5,10,15,20}, %指定x轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			ytick={0, 15,30,45,60,75}, %指定y轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			xlabel near ticks, % 设置x坐标名位置靠近折线图
			ylabel near ticks, % 设置y坐标名位置靠近折线图
			ymajorgrids=true, % 启用/禁用 [公式] 轴上刻度线位置上的网格线
			grid style=dashed, % 设置网格线格式
			legend style={at={(0.9,1.1)},anchor=south}, % 设置标签位置
%			legend columns=3, %设置标签列数
%			legend pos=north west, % 设置折线对应标签的位置
%			legend style={nodes={scale=0.6, transform shape}},  % 设置折线标签的格式
			]
			
			%画第一条线，semithick设置线的粗细为0.6pt，mark是折线标示形状，options是mark形状的大小 ， olive!50!white是颜色，coordinates中包含要绘制的点的坐标
			\addplot+[semithick,mark=x,mark options={scale=0.6}, color=color1] plot coordinates { 
				(0,66.58)
				(5,35.71)
				(10,38.99)
				(15,36.31)
				(20,42.19)
			};
			\addlegendentry{text-davinci-002}%第一条线标签
			
			%画第二条线
			\addplot+[semithick,mark options={scale=0.3}, color=color2] plot coordinates {
				(0,71.79)
				(5,50.74)
				(10,53.33)
				(15,56.67)
				(20,53.75)
			};
			\addlegendentry{code-davinci-002} %第二条线标签
			
			%画第三条线
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(0,72.53)
				(5,64.33)
				(10,59.05)
				(15,63.81)
				(20,71.25)
			};
			\addlegendentry{text-davinci-003} %第三条线标签


			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(0,32.53)
				(5,23.33)
				(10,13.05)
				(15,23.81)
				(20,44.25)
			};
			\addlegendentry{code-CodeRel} 


			\end{axis}
			\end{tikzpicture}



  }
		\caption{Analysis of Different  Prompt in CONLL04 } % 设置caption
		\label{fig:label}  % 设置用于reference的label
	\end{figure*}

% \end{document}


==> figures/old/few-shot.tex <==
% \documentclass[letterpaper]{article} % 
% \usepackage{pgfplots} % 画折线图
% \usepackage{scalefnt} %用于设置字体

% \definecolor{color1}{RGB}{145,30,180}
% \definecolor{color2}{RGB}{245,130,48}
% \definecolor{color3}{RGB}{230,25,75}

% \begin{document}
	
	\begin{figure}[h] %插入图片
		\centering %图片居中
		\resizebox{0.8\columnwidth}{!}{  %用于修改图片大小
			\begin{tikzpicture} %tikz图片
			\scalefont{0.7} %设置字体大小
			\begin{axis}[
			sharp plot, %控制线的风格
			title=line chart,%图像标题
			xmode=normal,% 控制坐标轴为线性
%		ymode=log,% 控制坐标轴为对数
			xlabel=x, %x坐标名
			ylabel=y, %y坐标名
			width=8cm, height=5cm,  %设置长和宽
			xmin=0,xmax=20,  % 设置x坐标范围
			ymin=30, ymax=80,  % 设置y坐标范围
			xtick={0,5,10,15,20}, %指定x轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			ytick={30,45,60,75}, %指定y轴刻度值。如果为空，则自动设置刻度线。即分割坐标轴
			xlabel near ticks, % 设置x坐标名位置靠近折线图
			ylabel near ticks, % 设置y坐标名位置靠近折线图
			ymajorgrids=true, % 启用/禁用 [公式] 轴上刻度线位置上的网格线
			grid style=dashed, % 设置网格线格式
			legend style={at={(0.9,1.1)},anchor=south}, % 设置标签位置
%			legend columns=3, %设置标签列数
%			legend pos=north west, % 设置折线对应标签的位置
%			legend style={nodes={scale=0.6, transform shape}},  % 设置折线标签的格式
			]
			
			%画第一条线，semithick设置线的粗细为0.6pt，mark是折线标示形状，options是mark形状的大小 ， olive!50!white是颜色，coordinates中包含要绘制的点的坐标
			\addplot+[semithick,mark=x,mark options={scale=0.6}, color=color1] plot coordinates { 
				(0,66.58)
				(5,35.71)
				(10,38.99)
				(15,36.31)
				(20,42.19)
			};
			\addlegendentry{a}%第一条线标签
			
			%画第二条线
			\addplot+[semithick,mark options={scale=0.3}, color=color2] plot coordinates {
				(0,71.79)
				(5,50.74)
				(10,53.33)
				(15,56.67)
				(20,53.75)
			};
			\addlegendentry{b} %第二条线标签
			
			%画第三条线
			\addplot+[semithick,mark options={scale=0.3}, color=color3] plot coordinates {
				(0,72.53)
				(5,64.33)
				(10,59.05)
				(15,63.81)
				(20,71.25)
			};
			\addlegendentry{c} %第三条线标签

			\end{axis}
			\end{tikzpicture}
		}
		\caption{Few-shot} % 设置caption
		\label{fig:label}  % 设置用于reference的label
	\end{figure}

% \end{document}


==> old/Results_cross_re.tex <==


\begin{table*}[t]
	\centering

	\scalebox{1.0}{
			% \begin{tabular}{@{}l ccc ccc ccc ccc ccc ccc@{}}
			% 	\toprule[2pt]
			% 	\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{News \faNewspaper} & \multicolumn{3}{c}{Politics} & \multicolumn{3}{c}{AI} & \multicolumn{3}{c}{Music} & \multicolumn{3}{c}{Literature} & \multicolumn{3}{c}{Science} \\ 
			% 	\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} \cmidrule(l){11-13}  \cmidrule(l){14-16} \cmidrule(l){17-19} 
			% 	\multicolumn{2}{c}{} P  & R  & F1 & P & R & F1 & P & R & F1  & P & R & F1  & P & R & F1 & P & R & F1\\  
			% 	\midrule
			% 	  TPlinker \cite{TPLinker} &  &  &  &  &  &  &  &  &  \\
   %  		     PRGC \cite{PRGC}&  &  &  &  &  &  &  &  &  \\
			% 	TANL \cite{TANL}  &  &  &  &  &  &  &  &  &  \\
			% 	UIE \cite{UIE} &  &  &  &  &  &  &  &  &  \\
			% 	% RelationPrompt &  &  &  &  &  &  &  &  &  \\
			% 	\midrule[0.1pt]
			% 	\textbf{CodeRel\_base} &  &  &  &  &  &  &  &  &  \\
   %  		    \textbf{CodeRel\_large} &  &  &  &  &  &  &  &  &  \\
			% 	\bottomrule[2pt]
			% \end{tabular}
            \begin{tabular}{lllllll}
            \toprule
            Model & \faNewspaper & \faLandmark  & \faLeaf & \faMusic & \faBookOpen & \faRobot \\
            \midrule
            TPlinker \cite{TPLinker} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
            PRGC \cite{PRGC} & 0.00 & 0.00 & 0.00 &0.00  & 0.00 & 0.00 \\
            TANL \cite{TANL} & 11.53 & 17.21 & 11.77 & 20.54 & 20.36 & 14.57 \\
            % UIE \cite{UIE} & 29.46 & 36.64 & 31.22 & 45.83 & 41.94 & 31.84 \\
            % \midrule
             ASP \cite{ERE} &  &  &  &  &  &  \\
            % \midrule
            % \textbf{CodeRel\_base}  &  &  &  &  &  &  \\
            \textbf{CodeRel} & {10.80} & {24.95} & {17.58} & {30.86} & {27.96} & { 20.09} \\
            \bottomrule
            \end{tabular}
	}
	\caption{
    F1-score (\%) of our proposed Code4Rel and baselines on cross domain settings.
	We select the dataset which includes the following domains: news (\faNewspaper), politics (\faLandmark), natural science (\faLeaf), music (\faMusic), literature (\faBookOpen) and artificial intelligence (\faRobot; AI).
	}
    \label{tab:cross}
 
\end{table*}

% 两个数据集music; ai; 17种关系?; 
% 现在triple_list没有到17种

% ai
% 1-shot, 5-shot, 10-shot(已经有结果)
% music
% 1-shot, 5-shot, full(已经有结果)


==> old/Results_small.tex <==

% \begin{table*}[t]
% \centering
% \begin{tabular}{ll ccc ccc}
% \toprule
% & \multirow{2}{*}{\textbf{Model} } & \multicolumn{3}{c}{\textbf{20-Shot}} & \multicolumn{3}{c}{\textbf{Full}} \\ \cline{3-8}
%  &  & \textbf{P}  & \textbf{R} & \textbf{F1}  & \textbf{P}  & \textbf{R} & \textbf{F1}   \\ 
% \multirow{2}{*}{\textbf{Not Pre-trained} } &  {CodeRel-text} &  &  &   \\
% & {CodeRel-code} &  &  &  \\ 
% \midrule
% \multirow{2}{*}{\textbf{Pre-trained} }& {CodeRel-text}  &  &  &  \\
% & {CodeRel-code} &  &  &  \\
% \bottomrule
% \end{tabular}
% \caption{CoNLL04, base}
% \end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{ll ccc}
\toprule
& \multirow{2}{*}{\textbf{Model} } & \multicolumn{3}{c}{\textbf{CONLL04}} \\ \cline{3-5}
 &  & \textbf{P}  & \textbf{R} & \textbf{F1}   \\ 
\midrule
\multirow{2}{*}{\textbf{Not Pre-trained} } &  {CodeRel-text} &  &  &   \\
& {CodeRel-code} &  &  &  \\ 
\midrule
\multirow{2}{*}{\textbf{Pre-trained} }& {CodeRel-text}  &  &  &  \\
& {CodeRel-code} &  &  &  \\
\bottomrule
\end{tabular}
\caption{CoNLL04, base}
\end{table*}

==> old/Results_triple_extraction_bak.tex <==


\begin{table}[!ht]
\footnotesize
\centering
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{lcc}
\toprule
\textbf{Method} & NER & RE\\
\midrule
\multicolumn{3}{l}{\textbf{NYT $\vartriangle$}} \\
CopyRE \text{ \citep{zeng-etal-2018-extracting}} & 86.2 & 58.7 \\
GraphRel \text{\ \citep{fu-etal-2019-graphrel}} & 89.2 & 61.9 \\
CopyRL \citep{zeng-etal-2019-learning} & - & 72.1 \\
Casrel \text{\ \citep{wei-etal-2020-novel}} $^{\dag}$ & (93.5) & 89.6 \\ 
TpLinker \citep{wang-etal-2020-tplinker} $^{\dag}$ & - & 91.9 \\
PFN \cite{DBLP:conf/emnlp/YanZFZW21} $^{\dag}$  & 95.8 & 92.4 \\
%UIE \cite{UIE}& &93.5 
\hline
\textbf{CodeRel} & 94.9 & 90.0 \\
\midrule
\multicolumn{3}{l}{\textbf{WebNLG $\vartriangle$}} \\
CopyRE \text{ \citep{zeng-etal-2018-extracting}} & 82.1 & 37.1 \\
GraphRel \text{\ \citep{fu-etal-2019-graphrel}} & 91.9 & 42.9 \\
CopyRL \citep{zeng-etal-2019-learning} & - & 61.6 \\
Casrel \text{\ \citep{wei-etal-2020-novel}} $^{\dag}$ & (95.5) & 91.8 \\ 
TpLinker \citep{wang-etal-2020-tplinker} $^{\dag}$ & - & 91.9 \\
PFN \cite{DBLP:conf/emnlp/YanZFZW21} $^{\dag}$ & 98.0 & 93.6 \\
%UIE \cite{UIE}&  & 2.66 \\ 
\hline
\textbf{CodeRel} & 95.9 & 89.8\\
\midrule
\multicolumn{3}{l}{\textbf{ADE $\blacktriangle$}} \\
Multi-head \citep{bekoulis2018joint} & 86.4 & 74.6 \\
Multi-head + AT \citep{bekoulis2018adversarial} & 86.7 & 75.5 \\
Rel-Metric \citep{tran2019neural} & 87.1 & 77.3 \\
SpERT \citep{eberts2019span} $^{\dag}$ & 89.3 & 79.2 \\
Table-Sequence \citep{wang-lu-2020-two} $^{\ddag}$ & 89.7 & 80.1 \\
%PFN$^{\dag}$ & 89.6 & 80.0 \\
PFN \cite{DBLP:conf/emnlp/YanZFZW21} $^{\ddag}$ & 91.3 & 83.2 \\
%UIE \cite{UIE}&  & 81.8 \\ 
\hline
\textbf{CodeRel} && \\
\midrule
\multicolumn{3}{l}{\textbf{ACE05} $\vartriangle$} \\
Structured Perceptron \citep{li-ji-2014-incremental} & 80.8 & 49.5 \\ 
SPTree \citep{miwa-bansal-2016-end} & 83.4 & 55.6 \\
Multi-turn QA \citep{li-etal-2019-entity} $^{\dag}$ & 84.8 & 60.2 \\
Table-Sequence \citep{wang-lu-2020-two} $^{\ddag}$ & 89.5 & 64.3 \\
PURE \citep{zhong2021frustratingly} $^{\ddag}$ & 89.7& 65.6 \\
\hline
PFN \cite{DBLP:conf/emnlp/YanZFZW21} $^{\ddag}$ & 89.0 & 66.8 \\
%UIE \cite{UIE}& 89.2 & 67.9 \\ 
\hline
\textbf{CodeRel} && \\
\midrule
\multicolumn{3}{l}{\textbf{SciERC} $\vartriangle$} \\
SPE \citep{wang-etal-2020-pre} $^{\S}$ & 68.0 & 34.6 \\
PURE \citep{zhong2021frustratingly} $^{\S}$ & 66.6 & 35.6 \\
PFN \cite{DBLP:conf/emnlp/YanZFZW21}  $^{\S}$ &66.8 &38.4\\
%UIE \cite{UIE}   & & \\ \hline
\textbf{CodeRel} && \\
\bottomrule
\end{tabular}
}
\caption{Experiment results on six datasets.
$^{\dag}$, $^{\ddag}$ and $^{\S}$ denotes the use of BERT, ALBERT and SCIBERT pre-trained embedding.
% \citep{devlin2019bert, Lan2020ALBERT:, beltagy-etal-2019-scibert}
% $\vartriangle$ and $\blacktriangle$ denotes the use of micro-F1 and macro-F1 score. NER results of Casrel are its reported average score of head and tail entity. Results of PURE are reported in single-sentence setting for fair comparison.
}
\label{tab:full-supervise}
% \vspace{-3.5mm}
\end{table}

==> old/Statistics_dataset.tex <==
c\begin{table}[ht]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{@{}lcccc@{}}
        \toprule[2pt]
        \multicolumn{1}{l}{\multirow{2}{*}{Category}} & \multicolumn{4}{c}{Dataset} \\ 
        \cmidrule(l){2-5}
        \multicolumn{1}{l}{} & Train & Valid   & Test   & Relations  \\ 
        \midrule
        WebNLG & & & &      \\
        ACE05 & & & &     \\
        SCIERC & & & &     \\
        CONLL04 & & & &    \\ 
        \bottomrule[2pt]
    \end{tabular}
    }
    \caption{Statistics of datasets. 
    $N$ is the number of triples in a sentence, E-len denotes the maximum length of entities using byte pair encoding (BPE), which determines the setting of the hyper-parameter $C$ (the length of candidate entities). }
    % \label{tab:dataset}
\end{table}

==> old/Statistics_dataset_cross_re.tex <==
\begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|ccc|c|ccc|c}
    \toprule
    & \multicolumn{4}{c|}{\textsc{sentences}} & \multicolumn{4}{c}{\textsc{relations}} \\
    \midrule
    & train & dev & test & \textbf{tot.} & train & dev & test & \textbf{tot.} \\
    \midrule
    Newspaper & 164 & 350 & 400 & 914 & 175 & 300 & 396 & 871 \\
    Landmark & 101 & 350 & 400 & 851 & 502 & 1,616 & 1,831 & 3,949 \\
    Leaf & 103 & 351 & 400 & 854 & 355 & 1,340 & 1,393 & 3,088 \\
    Music & 100 & 350 & 399 & 849 & 496 & 1,861 & 2,333 & 4,690 \\
    BookOpen & 100 & 400 & 416 & 916 & 397 & 1,539 & 1,591 & 3,527 \\
    Robot & 100 & 350 & 431 & 881 & 350 & 1,006 & 1,127 & 2,483 \\
    \midrule
    \textbf{tot.} & 668 & 2,151 & 2,446 & \textbf{5,265} & 2,275 & 7,662 & 8,671 & \textbf{18,608} \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Statistics.} Number of sentences and number of relations annotated for each domain.
    }
\end{table}

==> old/Statistics_dataset_pre-train.tex <==
\begin{table}[t]
\centering
% \footnotesize
% \renewcommand\tabcolsep{4.5pt}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{lllll}
\toprule[1.2pt]
% \toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sentences}} &  \multirow{2}{*}{\makecell[l]{\textbf{Triples}} } & \multirow{2}{*}{\textbf{Relations}}  \\ 
&&&& \\
\midrule
T-REx~ & 838,821  &  4,378,318 & 10,496  \\

TEKGEN~ & 6,310,061 & 10,609,697 &  1,013 \\

KELM~ & 15,616,551  & 35,117,608  &  59,904 \\

\midrule
Overall ~ & 22,765,433  & 50,105,623 & 71,413 \\ 
\bottomrule[1.2pt]
% \bottomrule
\end{tabular}
}
\caption{{Pre-training dataset statistics and corresponding pre-training tasks. \#Sent. and \#Rel. denote the number of sentences and relations respectively.}}
\label{tab:ptdata}
\end{table}

==> old/bak.tex <==
% \begin{table*}[t]
% 	\centering

% 	\scalebox{1.0}{
% 			\begin{tabular}{@{}l ccc ccc ccc@{}}
% 				\toprule[2pt]
% 				\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{WebNLG} & \multicolumn{3}{c}{SCIREC} & \multicolumn{3}{c}{CoNLL04} \\ 
% 				\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} 
% 				\multicolumn{2}{c}{} P  & R  & F1 & P & R & F1 & P & R & F1 \\  
% 				\midrule 
% 				Prompt-based zero-shot $\dag$ &  &  &  &  &  &  &  &  &  \\
% 				\midrule
% 				UIE &  &  &  &  &  &  &  &  &  \\
% 				TANL  & 0.783 & 0.754 & 0.768 & 0.203 & 0.183 & 0.193 & 0.567 & 0.482 & 0.521 \\
% 				RelationPrompt &  &  &  &  &  &  &  &  &  \\
% 				\midrule[0.1pt]
% 				Code4Rel & 0.670 & 0.650 & 0.659 & 0.205 & 0.199 & 0.202 & 0.420 & 0.410 & 0.415 \\
% 				+  in-context prompt &  &  &  &  &  &  &  &  &  \\
% 		        +  xxx pre-training &  &  &  &  &  &  &  &  &  \\
% 				\midrule
% 				Fine-tuning(full) $\ddag$ &  &  &  &  &  &  &  &  &  \\				
% 				\bottomrule[2pt]
% 			\end{tabular}
% 	}
% 	\caption{Precision(\%), Recall (\%) and F1-score (\%) of our proposed Code4Rel and baselines.
% 	$\dag$ means no training examples are used;
% 	$\ddag$ full training set is used.
% 	}
% 	\label{tab:main}
% \end{table*}

% \begin{table*}[t]
% 	\centering

% 	\scalebox{1.0}{
% 			\begin{tabular}{@{}l ccc ccc ccc@{}}
% 				\toprule[2pt]
% 				\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{ACE05} & \multicolumn{3}{c}{SCIREC} & \multicolumn{3}{c}{CoNLL04} \\ 
% 				\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} 
% 				\multicolumn{2}{c}{} P  & R  & F1 & P & R & F1 & P & R & F1 \\  
% 				\midrule 
% 				Prompt-based zero-shot $\dag$ &  &  &  &  &  &  &  &  &  \\
% 				\midrule
% 				UIE &  &  &  &  &  &  &  &  &  \\
% 				TANL  &  &  &  & 0.203 & 0.183 & 0.193 & 0.557 & 0.476 & 0.513 \\
% 				RelationPrompt &  &  &  &  &  &  &  &  &  \\
% 				\midrule[0.1pt]
% 				Code4Rel &  &  &  & 0.237 & 0.223 & 0.230 & 0.386 & 0.370 & 0.377 \\
% 				+  in-context prompt &  &  &  &  &  &  &  &  &  \\
% 		        +  xxx pre-training &  &  &  &  &  &  &  &  &  \\
% 				\midrule
% 				Fine-tuning(full) $\ddag$ &  &  &  &  &  &  &  &  &  \\				
% 				\bottomrule[2pt]
% 			\end{tabular}
% 	}
% 	\caption{Precision(\%), Recall (\%) and F1-score (\%) of our proposed Code4Rel and baselines.
% 	$\dag$ means no training examples are used;
% 	$\ddag$ full training set is used.
% 	}
% 	\label{tab:main}
% \end{table*}


\begin{table*}[t]
	\centering

	\scalebox{1}{
			% \begin{tabular}{@{}l ccc ccc ccc@{}}
			% 	\toprule[2pt]
			% 	\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{ADE} & \multicolumn{3}{c}{WebNLG} & \multicolumn{3}{c}{CoNLL04} \\ 
			% 	\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} 
			% 	\multicolumn{2}{c}{} P  & R  & F1 & P & R & F1 & P & R & F1 \\  
			% 	\midrule 
			% 	Prompt-based zero-shot $\dag$ &  &  &  &  &  &  &  &  &  \\
   %              "GPT3-Codex" in context learning &  &  &  &  &  &  &  &  &  \\
   %              % Fine-tuning &  &  &  &  &  &  &  &  &  \\
   %              \midrule
   %              RelationPrompt \cite{RelationPrompt} &  &  &  &  &  &  &  &  &  \\
			% 	UIE \cite{UIE}  &  &  &  &  &  &  &  &  &  \\
			% 	TANL \cite{TANL}  & 0.64 & 0.25 & 0.36 & 0.76 & 0.76 & 0.76 & 0.56 & 0.48 & 0.51 \\
			% 	% \midrule[0.1pt]
			% 	% Unixcode &  &  &  & 0.650 & 0.685 & 0.667 & 0.386 & 0.370 & 0.377 \\
   %              \midrule
   %              % CodeT5 & 0.42 & 0.33 & 0.37 & 0.51* & 0.78 & 0.62 & 0.31* & 0.45 & 0.37  \\  
   %              % \midrule
		 %        % Code4Rel &  &  &  & 0.68 & 0.79 & 0.69 &  &  &  \\
		 %        % +  in-context prompt &  &  &  &  &  &  &  &  &  \
   %              % \midrule
   %              % + large &  &  &  & 0.75  & 0.78 & 0.77  &  &  &  \\ 
   %              Code4Rel &  &  &  & 0.68 & 0.79 & 0.69 &  &  &  \\
			% 	\midrule
			% 	Fine-tuning(full) $\ddag$ &  &  &  &  &  &  &  &  &  \\			
			% 	\bottomrule[2pt]
			% \end{tabular}

			% \begin{tabular}{@{}lcccccc@{}}
			% 	\toprule[2pt]
			% 	\multicolumn{1}{c}{\multirow{2}{*}{Model}} & CoNLL04  & ADE  & ACE05  & WebNLG &  NYT & Wiki80 \\ 
			% 	\cmidrule(l){2-7} 
			% 	\multicolumn{1}{c}{} & F1 &  F1 & F1 & F1 & F1 & F1\\  
			% 	\midrule 
			% 	Prompt-based zero-shot $\dag$ &  &  &  &  &  & \\
   %              "Codex" in context learning  &  &  &  &  &  & \\
   %              % Fine-tuning &  &  &  &  &  &  &  &  &  \\
   %              \midrule
   %              TPlinker \cite{} &  &  &  &  &  & \\
   %              PRGC \cite{} &  &  &  &  &  &  \\
   %              TANL \cite{} &  &  &  &  &  &  \\
   %  	    UIE \cite{UIE} &  &  &  &  &  & \\
		 %    \textbf{CodeRel\_base}  &  &  &  &  &  & \\
   %  	     \textbf{CodeRel\_large}  &  &  &  &  &  & \\
			% 	\midrule
   %              Tplinker \cite{} &  &  &  &  &  & \\
   %              PRGC \cite{} &  &  &  &  &  &  \\
   %              TANL \cite{} &  &  &  &  &  &  \\
   %  	    UIE \cite{UIE} &  &  &  &  &  & \\
		 %    \textbf{CodeRel\_base}  &  &  &  &  &  & \\
   %  	    \textbf{CodeRel\_large}  &  &  &  &  &  & \\
			% 	\bottomrule[2pt]
			% \end{tabular}

   % 			\begin{tabular}{@{}lcccccc@{}}
			% 	\toprule[2pt]
			% 	\multicolumn{1}{c}{\multirow{2}{*}{Model}} & CoNLL04  & ADE  & ACE05  & WebNLG &  NYT & Wiki80 \\ 
			% 	\cmidrule(l){2-7} 
			% 	\multicolumn{1}{c}{} & F1 &  F1 & F1 & F1 & F1 & F1\\  
			% 	\midrule 
			% 	Prompt-based zero-shot $\dag$ &  &  &   \\
   %              "Codex" in context learning  &  &  &  \\
   %              % Fine-tuning &  &  &  &  &  &  &  &  &  \\
   %              \midrule
   %              TPlinker \cite{} &  &  &  \\
   %              PRGC \cite{} &  &  &   \\
   %              TANL \cite{} &  &  &    \\
   %  	    UIE \cite{UIE} &  &  &   \\
		 %    \textbf{CodeRel\_base}  &  &  &  \\
   %  	     \textbf{CodeRel\_large}  &  &  &  \\
			% 	\midrule
   %              Tplinker \cite{} &  &  &   \\
   %              PRGC \cite{} &  &  &    \\
   %              TANL \cite{} &  &  &  &  &  &  \\
   %  	    UIE \cite{UIE} &  &  &  &  &  & \\
		 %    \textbf{CodeRel\_base}  &  &  &  &  &  & \\
   %  	    \textbf{CodeRel\_large}  &  &  &  &  &  & \\
			% 	\bottomrule[2pt]
			% \end{tabular}

   % 			\begin{tabular}{@{}l ccc ccc ccc@{}}
			% 	\toprule[2pt]
			% 	\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{3}{c}{CoNLL04}  & \multicolumn{3}{c}{ADE}  & \multicolumn{3}{c}{ACE05} \\ 
			% 	\cmidrule(l){2-10} 
			% 	\multicolumn{1}{c}{} & P & R & F1 & P & R & F1 & P & R & F1\\  
			% 	\midrule 
			% 	Prompt-based zero-shot $\dag$ &  &  &   \\
   %              "Codex" in context learning  &  &  &  \\
   %              % Fine-tuning &  &  &  &  &  &  &  &  &  \\
   %              \midrule
   %              TPlinker \cite{TPLinker} &  &  &  \\
   %              PRGC \cite{PRGC} &  &  &   \\
   %              TANL \cite{TANL} &  &  &    \\
   %  	    UIE \cite{UIE} &  &  &   \\
   %       \midrule
		 %    \textbf{CodeRel\_base}  &  &  &  \\
   %  	     \textbf{CodeRel\_large}  &  &  &  \\
			% 	\midrule
   %              TPlinker \cite{TPLinker} &  &  &   \\
   %              PRGC \cite{PRGC} &  &  &    \\
   %              TANL \cite{TANL} &  &  &  &  &  &  \\
   %  	    UIE \cite{UIE} &  &  &  &  &  & \\
   %       \midrule
		 %    \textbf{CodeRel\_base}  &  &  &  &  &  & \\
   %  	    \textbf{CodeRel\_large}  &  &  &  &  &  & \\
			% 	\bottomrule[2pt]
			% \end{tabular}

\iffalse

% 本表废弃
\begin{tabular}{lccccccccc}
\toprule
Model & \multicolumn{3}{c}{CoNLL04} & \multicolumn{3}{c}{ADE} & \multicolumn{3}{c}{SciERC} \\ \cline{2-10} 
& P & R & F1 & P & R & F1 & P & R & F1 \\
\midrule
%\multirow{2}{*}{Zero shot learning} & Prompt-based zero-shot &  &  &  &  &  &  &  &  &  \\
% & "Codex" in context learning &  &  &  &  &  &  &  &  &  \\
%\midrule
%\multirow{6}{*}{ Few shot learning} &  TPlinker \cite{TPLinker} &  &  &  &  &  &  &  &  &  \\
% & PRGC \cite{PRGC} &  &  &  &  &  &  &  &  & \\
%  & TANL \cite{TANL} & 0.56 & 0.48 & 0.52  & 0.65 & 0.25 & 0.36 & 0.38 & 0.32 & 0.34     \\
%   & UIE \cite{UIE} &  &  &  &  &  &  &  &  & \\
 %   & PRGC \cite{PRGC} &  &  &  &  &  &  &  &  & \\ \cline{2-11} 
  %      & \textbf{CodeRel\_base} &  &  &  &  &  &  &  &  & \\
   %         & \textbf{CodeRel\_large} &  &  &  &  &  &  &  &  & \\
 %\midrule
 
DYGIE++ &  &  &  &  &  &  &  &  &  \\
TPlinker \cite{TPLinker} &  &  &  &  &  &  &  &  &  \\
PRGC \cite{PRGC} &  &  &  &  &  &  &  &  & \\
TANL \cite{TANL} &  &  &  &  &  &  &  &  & \\
UIE \cite{UIE} &  &  &  &  &  &  &  &  & \\

    \midrule
    \textbf{CodeRel} &  &  &  &  &  &  &  &  & \\
\bottomrule
\end{tabular}


	}
	\caption{Precision(\%), Recall (\%) and F1-score (\%) of our proposed Code4Rel and baselines.
	$\dag$ means no training examples are used;
	$\ddag$ full training set is used.
	}
	% \label{tab:main}
\end{table*}
\fi

\begin{table}[!ht]
\footnotesize
\centering
\begin{spacing}{1.19}
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{lcc}
\toprule
\textbf{Method} & NER & RE\\
\midrule
\multicolumn{3}{l}{\textbf{NYT $\vartriangle$}} \\
CopyRE \text{ \citep{zeng-etal-2018-extracting}} & 86.2 & 58.7 \\
GraphRel \text{\ \citep{fu-etal-2019-graphrel}} & 89.2 & 61.9 \\
CopyRL \citep{zeng-etal-2019-learning} & - & 72.1 \\
Casrel \text{\ \citep{wei-etal-2020-novel}} $^{\dag}$ & (93.5) & 89.6 \\ 
TpLinker \citep{wang-etal-2020-tplinker} $^{\dag}$ & - & 91.9 \\
PFN & \textbf{95.8} & \textbf{92.4} \\
\midrule
\multicolumn{3}{l}{\textbf{WebNLG $\vartriangle$}} \\
CopyRE \text{ \citep{zeng-etal-2018-extracting}} & 82.1 & 37.1 \\
GraphRel \text{\ \citep{fu-etal-2019-graphrel}} & 91.9 & 42.9 \\
CopyRL \citep{zeng-etal-2019-learning} & - & 61.6 \\
Casrel \text{\ \citep{wei-etal-2020-novel}} $^{\dag}$ & (95.5) & 91.8 \\ 
TpLinker \citep{wang-etal-2020-tplinker} $^{\dag}$ & - & 91.9 \\
\hline
PFN$^{\dag}$ & \textbf{98.0} & \textbf{93.6} \\
\midrule
\multicolumn{3}{l}{\textbf{ADE $\blacktriangle$}} \\
Multi-head \citep{bekoulis2018joint} & 86.4 & 74.6 \\
Multi-head + AT \citep{bekoulis2018adversarial} & 86.7 & 75.5 \\
Rel-Metric \citep{tran2019neural} & 87.1 & 77.3 \\
SpERT \citep{eberts2019span} $^{\dag}$ & 89.3 & 79.2 \\
Table-Sequence \citep{wang-lu-2020-two} $^{\ddag}$ & 89.7 & 80.1 \\
\hline
PFN$^{\dag}$ & 89.6 & 80.0 \\
PFN$^{\ddag}$ & \textbf{91.3} & \textbf{83.2} \\
\midrule
\multicolumn{3}{l}{\textbf{ACE05} $\vartriangle$} \\
Structured Perceptron \citep{li-ji-2014-incremental} & 80.8 & 49.5 \\ 
SPTree \citep{miwa-bansal-2016-end} & 83.4 & 55.6 \\
Multi-turn QA \citep{li-etal-2019-entity} $^{\dag}$ & 84.8 & 60.2 \\
Table-Sequence \citep{wang-lu-2020-two} $^{\ddag}$ & 89.5 & 64.3 \\
PURE \citep{zhong2021frustratingly} $^{\ddag}$ & \textbf{89.7} & 65.6 \\
\hline
PFN$^{\ddag}$ & 89.0 & \textbf{66.8} \\
\midrule
\multicolumn{3}{l}{\textbf{ACE04} $\vartriangle$} \\
Structured Perceptron \citep{li-ji-2014-incremental} & 79.7 & 45.3 \\ 
SPTree \citep{miwa-bansal-2016-end} & 81.8 & 48.4 \\
Multi-turn QA \citep{li-etal-2019-entity} $^{\dag}$ & 83.6 & 49.4 \\
Table-Sequence \citep{wang-lu-2020-two} $^{\ddag}$ & 88.6 & 59.6 \\
PURE \citep{zhong2021frustratingly} $^{\ddag}$ & 88.8 & 60.2 \\
\hline
PFN$^{\ddag}$ & \textbf{89.3} & \textbf{62.5} \\
\midrule
\multicolumn{3}{l}{\textbf{SciERC} $\vartriangle$} \\
SPE \citep{wang-etal-2020-pre} $^{\S}$ & \textbf{68.0} & 34.6 \\
PURE \citep{zhong2021frustratingly} $^{\S}$ & 66.6 & 35.6 \\
\hline
PFN$^{\S}$ &66.8 &\textbf{38.4} \\
\bottomrule
\end{tabular}
}
\end{spacing}
\caption{Experiment results on six datasets. $^{\dag}$, $^{\ddag}$ and $^{\S}$ denotes the use of BERT, ALBERT and SCIBERT\citep{devlin2019bert, Lan2020ALBERT:, beltagy-etal-2019-scibert} pre-trained embedding. $\vartriangle$ and $\blacktriangle$ denotes the use of micro-F1 and macro-F1 score. NER results of Casrel are its reported average score of head and tail entity. Results of PURE are reported in single-sentence setting for fair comparison.}
\label{tab:my-table2}
% \vspace{-3.5mm}
\end{table}

==> old/comparison.tex <==
\begin{table}[t]
\centering
% \footnotesize
% \renewcommand\tabcolsep{4.5pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ll}
\toprule
Work & Language Template \\
\midrule
TANL & \textbf{[ entity | type ]}  text \textbf{[ entity | type | relation ]} text \\

UIE & \textbf{<spot>} entity \textbf{<asoc>} relation \textbf{<text>} text\\

\midrule
CodeRel & \textbf{DocStrings} Class \textbf{Triple (Type) : Relation(entities)} \\ 
\bottomrule
% \bottomrule
\end{tabular}
}
\caption{Example of language templates for Relational Triple Extraction}
% \label{tab:ptdata}
\end{table}

==> tables/main.tex <==
\begin{table}[t]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{llcc}
\specialrule{0em}{1pt}{1pt}
\toprule
& \multirow{2}{*}{\textbf{Comparable SOTA} } & \multicolumn{2}{c}{\textbf{Dataset}} \\ \cline{3-4}
 &  & \textbf{ADE}  & \textbf{CONLL04}   \\ 
\midrule
% 
\multirow{2}{*}{{\textbf{Zero-Shot}} } & \cite{UIE} & 0 & 0    \\
% & CodeRel & 45.0  & 14.2 \\ 
& CodeRel & 19.1  & 4.1 \\ 
\midrule

% 3-shot
\multirow{2}{*}{\textbf{Few-Shot} }&  \cite{UIE}  & 50.3 & 39.0  \\
& {CodeRel} & 60.5 & 35.6 \\ 

% % 1-shot
% \multirow{2}{*}{\textbf{Few-Shot} }&  \cite{UIE}  & 28.1 & 36.5  \\
% & {CodeRel} & 46.7 & 17.9 \\ 


\midrule
\multirow{1}{*}{\textbf{Full} }&  \cite{UIE}  & 81.1 & 76.2    \\


\bottomrule
\end{tabular}
}
\caption{Performance of {\ours} and UIE \cite{UIE} with large LM (relation strict micro F1).}
\label{main-table}
\end{table}
% \multirow{2}{*}{\textbf{Few-Shot} }&  \cite{UIE}  & 49.7 & 43.5  \\
% & {CodeRel} & 40.0 & 22.7  \\ 
% & {CodeRel} &  &   \\ 

==> tables/table.tex <==
% \begin{table*}[t]
% \centering
% \begin{tabular}{llccc}
% \toprule
% & \multirow{2}{*}{\textbf{Comparable SOTA} } & \multicolumn{2}{c}{\textbf{Dataset}} \\ \cline{3-5}
%  &  & \textbf{ADE}  & \textbf{CONLL04}  & \textbf{SciERC}  \\ 
% \midrule

% \multirow{1}{*}{{\textbf{Zero-Shot}} } 
% & Vanilla Prompt (code-davinci-002) & 10.3  & ? & \\ 
% & Vanilla Prompt (text-davinci-002) &   &  &  \\
% \cline{2-5}
% & CodeKGC (code-davinci-002) & 19.1 & 4.1 & \\ 
% & CodeKGC (text-davinci-002) &  &  & \\ 
% \midrule

% \multirow{2}{*}{\textbf{Few-Shot} }
% & Vanilla Prompt (code-davinci-002) & 44.6 & ? & ?\\ 
% & Vanilla Prompt (text-davinci-002) &  & & \\ 
% \cline{2-5}
% & CodeKGC (code-davinci-002) & 60.5 & 35.6 & ?\\ 
% & CodeKGC (text-davinci-002) &  &  &\\ 

% \bottomrule
% \end{tabular}
% % }
% \caption{Performance of {\ours} and baselines in 0-shot and few-shot(3-shot) settings (relation strict micro F1).
% \dag means textual prompt and \ddag means code prompt.
% }
% \label{main-table}
% \end{table*}


% \begin{table*}[t]
% \centering
% \begin{tabular}{llccc}
% \toprule
% & \multirow{2}{*}{\textbf{Comparable SOTA} } & \multicolumn{2}{c}{\textbf{Dataset}} \\ \cline{3-5}
%  &  & \textbf{ADE}  & \textbf{CONLL04}  & \textbf{SciERC}  \\ 
% \midrule

% \multirow{1}{*}{{\textbf{Zero-Shot}} } 
% & Vanilla Prompt (code-davinci-002) & 10.3  & ? & \\ 
% & Vanilla Prompt (text-davinci-002) &   &  &  \\
% \cline{2-5}
% & CodeKGC (code-davinci-002) & 19.1 & 4.1 & \\ 
% & CodeKGC (text-davinci-002) &  &  & \\ 
% \midrule

% \multirow{2}{*}{\textbf{Few-Shot} }
% & Vanilla Prompt (code-davinci-002) & 48.2  &  & \\ 
% & Vanilla Prompt (text-davinci-002) & 50.7 & ? & \\ 
% \cline{2-5}
% & CodeKGC (code-davinci-002) & \textbf{65.4} & 30.7 & \\ 
% & CodeKGC (text-davinci-002) & 62.3  &  &\\ 

% \bottomrule
% \end{tabular}
% % }
% \caption{Performance of {\ours} and baselines in 0-shot and few-shot settings (relation strict micro F1).
% \dag means textual prompt and \ddag means code prompt.
% For few-shot setting, we choose 5-shot relation setting as demonstrations.
% For zero-shot setting, we replace relations with their synonyms.
% }
% \label{main-table}
% \end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{llccc}
% \toprule
% & \multirow{2}{*}{\textbf{Comparable SOTA} } & \multicolumn{2}{c}{\textbf{Dataset}} \\ \cline{3-5}
%  &  & \textbf{ADE}  & \textbf{CONLL04}  & \textbf{SciERC}  \\ 
% \midrule

% \multirow{1}{*}{{\textbf{Zero-Shot}} } 
% & Vanilla Prompt (text-davinci-002) &  &  & \\ 
% & Vanilla Prompt (text-davinci-003) &   &  &  \\
% \cline{2-5}
% & CodeKGC (text-davinci-002) &  &  & \\ 
% & CodeKGC (text-davinci-003) &  &  & \\ 
% \midrule

% \multirow{2}{*}{\textbf{Few-Shot} }
% & Vanilla Prompt (text-davinci-002) & 50.7 & 30.7  & 13.5  \\ 
% & Vanilla Prompt (text-davinci-003) & 54.4 & 43.4 & 20.2 \\ 
% \cline{2-5}
% & CodeKGC (text-davinci-002) & 62.3 & 31.5 & 13.5 \\ 
% & CodeKGC (text-davinci-003) & 65.1 & 37.1 & 18.5 \\ 

% \bottomrule
% \end{tabular}
% % }
% \caption{Performance of {\ours} and baselines in 0-shot and few-shot settings (relation strict micro F1).
% \dag means textual prompt and \ddag means code prompt.
% For few-shot setting, we choose 5-shot relation setting as demonstrations.
% For zero-shot setting, we replace relations with their synonyms.
% }
% \label{main-table}
% \end{table*}


